Neuro-Symbolic World Models for Adapting to Open World Novelty

Open-world novelty--a sudden change in the mechanics or properties of an environment--is a common occurrence in the real world. Novelty adaptation is an agent's ability to improve its policy performance post-novelty. Most reinforcement learning (RL) methods assume that the world is a closed, fixed process. Consequentially, RL policies adapt inefficiently to novelties. To address this, we introduce WorldCloner, an end-to-end trainable neuro-symbolic world model for rapid novelty adaptation. WorldCloner learns an efficient symbolic representation of the pre-novelty environment transitions, and uses this transition model to detect novelty and efficiently adapt to novelty in a single-shot fashion. Additionally, WorldCloner augments the policy learning process using imagination-based adaptation, where the world model simulates transitions of the post-novelty environment to help the policy adapt. By blending ''imagined'' transitions with interactions in the post-novelty environment, performance can be recovered with fewer total environment interactions. Using environments designed for studying novelty in sequential decision-making problems, we show that the symbolic world model helps its neural policy adapt more efficiently than model-based and model-based neural-only reinforcement learning methods.

==> 3_setting.tex <==

As is typical in reinforcement learning we model our environment as standard Markov decision processes (MDP): $M=\langle S, A, R, P, \gamma\rangle$, where
$S$ is the set of environment states, $A$ is the set of actions, $R:S \times A \rightarrow \mathbb{R}$ is the function mapping from states and actions to a scalar reward, $P:S \times A \rightarrow \mathbb{S}$ is the transition function between states, and $\gamma$ is the discount factor. 


The injection of novelty, after an arbitrary and {\em a priori} unknown number of episodes or games $t$ constitutes a transformation from the original environment or MDP $M$ to a new environment or MDP $M'$. 
% Given this model of environments, 
We consider all aspects of the problem except an agent's decision-making model to be property of the environment. 
This includes agent morphology, sensors, and action preconditions and effects. 
%
We assume that each agent's observation space and action space remain consistent before and after novelty is injected. 
This means that the  number of actions and the size and shape of observations are consistent throughout each experiment, but some never occur pre-novelty.
%
For example a volcano eruption is always a possibility, but it could be rare enough to be a singular experience with no previous occurrence; more prosaically, using a certain key to open a certain door is always a possibility, but it could have different outcome post-novelty, if the door has been re-keyed.
%
% This is consistent with a robotics perspective on MDPs, where actions and observations are governed by an underlying physics of the real world even if all possibilities are not observed, and carries over to our experiments within games and grid worlds~\cite{kejriwal2021multi,gamagenovelty}.
%
We also assume that the agent's mission $T$ is consistent before and after the novelty, meaning that we do not consider changes to the extrinsic agent rewards. 
% While changes to the goal and reward structure of an agent are indeed important in the real world, this is closely related to continual lifelong learning and multitask learning. 
% The integration of novelty adaptation with these fields is left to future work.





% \section{Fundamentals of Novelty Adaptation}

% \Mark{moved from intro} \jb{moved to setting}
% We distinguish between novelty and {\em continuous learning}, in which a learner makes the underlying assumption that some phenomenon is too complex to learn offline and a model must be continuously updated. 
% In contrast, novelty occurs suddenly and sporadically during test/deployment time.
% Novelty shares more similarity to {\em transfer learning} wherein a novelty can be thought of as transferring the agent to another environment that is nearly identical except in some small but non-trivial way.
% However, transfer learning often assumes that an agent can return to an offline training phase when encountering the new environment, whereas novelty adaptation must occur during execution in the environment.

% There are two main challenges to handling novelty. 
% The first is \em{novelty detection}.
% Learning during deployment is inefficient and harms performance if the world hasn't actually changed. 
% Thus, one may choose to have a separate process that monitors for novelty and then activates an adaptation process.
% The second challenge is \em{adaptation}.
% Once a novelty occurs, it is incumbent on the agent to restore its performance in as few steps as possible. 
% The naive approach to adaptation is to simply turn learning back on.
% It will take time for the policy to re-converge.
% {\em Model based} reinforcement learning, in which the agent learns a policy and the environment's latent transition function, can theoretically help because knowing the transition function can make policy learning more sample-efficient.
% However, the transition model must also be re-learned because novelty is a change in the environment dynamics; re-learning the transition model can also take many steps.



% \subsection{World Models in Reinforcement Learning}\label{sec:world_models_related}

% We model our environments as standard Markov decision processes (MDPs). As we operate in symbolically grounded domains we model sequential decision making problems as having two fundamentally different types of entities: agents and the environment, which we model as interacting in a stochastic game---a multi-agent generalization of MDPs. 
% The injection of novelty constitutes a transformation from the original game or MDP $M$ to a new game or MDP $M'$. 
% Given this model of environments, we consider all aspects of the problem except an agent's decision making model to be property of the environment. This includes agent morphology, sensors, and action preconditions and effects. 


% With this model of the environment we assume that each agent's observation space and action space remains consistent before and after novelty is injected. 
% The number of actions and the size and shape of observations are consistent throughout each experiment.

% This is consistent with a robotics perspective on MDPs where actions and observations are governed by an underlying physics of the real world, even though we experiment within grid worlds and games~\cite{kejriwal2021multi,gamagenovelty}.
% % \MarkLeft{added, not sure we should keep it}.

% Lastly, to focus on novelties emerging during the tasks, we assume that the agent's mission $T$ is consistent before and after the novelty, meaning that we do not consider changes to the extrinsic agent rewards. 
% While changes to the goal and reward structure of an agent are indeed important in the real world, this is closely related to continual lifelong learning and multitask learning. 
% The integration of novelty adaptation with these fields is left to future work.



% \subsection{Novelty in Sequential Decision Making Environments}\label{sec:nov_background}

% Novelty can be described in the context of differences in an environment over a period of time and associated capabilities to detect and respond to those changes~\cite{langley2020open}. 
% Boult et al.~\cite{boult2021towards} looks to unify the study of novelty both sequential decision making and traditional machine learning domains, categorizing novelties broadly as \textit{world novelties}, \textit{agent novelties}, and \textit{observation novelties}. 
% By Boult et al. definition, world novelties are changes in the objects and dynamics of the world external to the agent as well as the agent's abilities to affect change on the world.
% Agent novelties are those where the agent's state does not align with the agent's prior understanding of the world and/or can be classified by the agent as a novelty. 
% Observation novelties are those where a sense-making tool external to the agent (e.g., a sensor) is subject to changes in the environment, such as when a camera or radar signal experiences deterioration from use or unexpected interference. 





% % "What IS NOT novelty?"
% Novelty and novelty adaptation is not equivalent to research areas and methods related to outliers like outlier detection or rejection---outliers assumes \textit{a priori} some correct or expected distribution, where the points or behaviors that lie outside that distribution are aberrant behavior.
% By contrast, novelty is a sudden change that changes the environment distribution unexpectedly~\cite{chandola2007outlier}.

% Novelty adaptation is also different from {\em continual learning} or {\em lifelong learning}.
% In continual and lifelong learning there exists a sequence "tasks", each of which could be different environments, datasets, or novel classes. 
% These tasks can be overlapping, task boundaries don't have to be well-defined, and can include a mixture of supervised and unsupervised data, but in most cases these tasks are disjoint and task boundaries are known and discrete~\cite{parisi2019continual,silver2013lifelong,smith2021memory}. 
% Most distinctly, in continual learning the model is trained on only one task at a time but validated on that task and all prior tasks. 
% Novelty adaptation, on the other hand, only requires the agent to perform well at the task at hand, so before the introduction of the novelty the agent is evaluated only on the pre-novelty world and then only on post-novelty world after novelty is introduced.

% Novelty adaptation is a superset of domain shift and domain adaptation. 
% Domain adaptation in sequential decision making problems specifically addresses problems where training and deployment have the same feature space but different distributions over that feature space~\cite{zhang2019vr,sun2015survey}. 
% Additionally, this research domain usually assumes that the agent must adapt to this extremely quickly--few shot domain adaptation--or simply be robust to these changes--as in zero-shot domain adaptations. 
% By this definition, domain shift and domain adaptation are one aspect of novelty and novelty adaptation, but novelty goes beyond this by also including variation of the fundamental dynamics of an environment and the agent interactions as well. 

% % open set recognition....?

% The closest analog to novelty adaptation is transfer learning. Given a set of source or training tasks and a target task, transfer learning aims to learn an optimal policy for the target domain leveraging what it learned from the source domains as well as what it has access to in the target domain \cite{zhu2021transfer}. 
% While there are some works that focus on variants like zero-shot transfer learning--most notably research focused on transferring from a simulation to the real world--for the most part transfer learning studies the mechanics of model reuse and fine tuning~\cite{higgins2017darla}. 
% That is to say: given an already trained model trained on a certain task, how would one reuse this model in a new task where this new task can range from being a subtask of the original task to being completely unrelated. 
% In novelty adaptation on the other hand the pre-novelty and post-novelty tasks are always related by a (usually realistic) transformation. 
% While transfer learning optimizes the reuse of a learned model with no constraints on the relationship between source and target tasks and by any means necessary, novelty adaptation optimizes for adaptation performance and efficiency online given the knowledge that a realistic transformation between source and target exists. 



% Novelty could affect the environment as actions taking on different effects, or observations and states that never occur pre-novelty that start to occur post-novelty.


% % We expand upon the category of {\em world novelties}.
% % We further sub-divide world novelties along two dimensions. 
% Per \cite{balloch2022novgrid} we characterize novelties along three dimensions. 
% The first dimension is \textbf{object} vs \textbf{action} novelties.
% Objects are any component of the environment that is not controllable. 
% This includes keys, doors, balls, etc.
% Object novelties involve changes to, or the introduction or removal of, objects or classes of objects. 
% Actions are the ways in which the world is affected by controllable entities.
% Action novelties involve changes in the dynamics of actions through which the state of the world is affected. 
% Action novelties can involve changes in the preconditions of actions---the applicability criteria of actions---or action effects---the way in which the world is changed when an action is executed. 

% Second, novelties can be expressed as changes to \textbf{unary} predicates or \textbf{non-unary} (or $n$-ary where $n>1$) relations.
% Unary object novelties can be thought of as added, removed, or changes to intrinsic properties of objects like mass, volume, or shape. 
% Non-unary object novelties are changes in the relationship between objects, which is to say properties of objects that are necessarily defined in the context of other entities.
% Unary and non-unary action novelties involve 
% (a)~the addition, removal, or change of properties of objects required for action applicability, or 
% (b)~changes to the properties of objects or changes to the relationship between objects.

% Third, we observe that novelties can be categorized according to how they change the distribution of solutions to a task: 
%  \begin{itemize}
%      \item {\bf Barrier novelty}---the optima in the solution distribution are longer after novelty than before novelty.
%      For example: a door the agent must pass through to achieve a goal initially required one key pre-novelty but requires the agent to possess two keys simultaneously post-novelty.
%      \item {\bf Shortcut novelty}---the optima in the solution distribution are on average shorter after novelty than before novelty.
%      For example, a door that required a key pre-novelty then does not require any keys post-novelty.
%      \item {\bf Delta novelty}---the optima in the solution distribution are the same before and after novelty injection.
%      For example, a door that required one key pre-novelty then requires a different key post-novelty.
%     %  \item \Mark{Should we have distraction novelty here where a change does not affect the agent's optimal trajectory? If so, how do we distinguish from delta?} \jb{in the analogy of our ontology to a numeric system, distraction novelties are basically like our "zero". They are potentially worth talking about, but ultimately not necessary. I think we leave it for the future paper where we will be more important as we will be discussing novelty detection as well}
%  \end{itemize}

% \julia{....I think the section could end here with whatever below that can be merged into the above}
% \Mark{Merge with above:}

%  * Four axes of novelty:
 
%  ** Object Vs Action: objects are any component of the world that is not controllable. Actions are the ways in which the world is affected by controllable entities, which we call actors or agents.
 
%  ** Unary vs. Non-Unary: This refers to the relational properties of the objects affected by novelty. Unitary signifies any novelty that doesn't require more than one entity or action to be relevant, whereas non-unitary novelties do require more than one entity to be relevant. So, for example, a unitary object novelty might modify the weight or color of an object, and a unitary action novelty might modify the range of an actions applicability, like moving two twice as far forward with the same effort as before novelty. These can have some effect on other entities in the environment, but these changes are intrinsic to the action and objects independent of other entities. A non-unitary object novelty might be whether a key unlocks a door; indeed, the key geometry is fundamental to the key, however the fact that it can or cannot unlock a door is of no value without the existence of a door. Likewise, a non-unitary action novelty might be a change to whether an agent can walk through walls; again, while the fact of a wall being passable is an intrinsic property of the wall, the passability of a wall is irrelevant information without the existence of an agent that can (or cannot) pass through it.
 
%  ** Barrier vs. Shortcut vs. Delta solutions: This property of a novelty characterizes the way in which the solution distribution changes as a result of the novelty with respect to the decision trajectories that connect the start and the goal. Specifically, comparing the complete distribution of decisions that link the goal state and the initial state, 
%  \begin{itemize}
%      \item the novelty is a shortcut if the optima in the solution distribution are on average shorter after novelty than before novelty
%      \item the novelty is a barrier if the optima in the solution distribution are shorter after novelty than before novelty
%      \item the novelty is a delta if the optima in the solution distribution are shorter after novelty than before novelty
%  \end{itemize}
 


 


==> 8_ackn.tex <==

\section{Acknowledgements}

This research is sponsored in part by the Defense Advanced Research Projects Agency (DARPA), under contract number W911NF-20-2-0008. Views and conclusions contained in this document are those of the authors and should not be interpreted as necessarily representing official policies or endorsements, either expressed or implied, of the US Department of Defense or the United States Government.
We gratefully acknowledge David Aha, Katarina Doctor, and members of the DARPA SAIL-ON Working Group on Metrics.



==> 9_checklist.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

% \julia{My crummy LaTeX skills cannot make the section references work}

\begin{enumerate}


 \item For all authors...
 \begin{enumerate}
   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
     \answerYes{}
   \item Did you describe the limitations of your work?
     \answerYes{See Conclusions section.}
   \item Did you discuss any potential negative societal impacts of your work?
     \answerYes{See Conclusions section as well as the Societal Impacts section in the Appendix.}
   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
     \answerYes{}
 \end{enumerate}


 \item If you are including theoretical results...
 \begin{enumerate}
   \item Did you state the full set of assumptions of all theoretical results?
     \answerNA{}
         \item Did you include complete proofs of all theoretical results?
     \answerNA{}
 \end{enumerate}


 \item If you ran experiments...
 \begin{enumerate}
   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
     \answerYes{Repository link will be included in de-anonymized version}
   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
     \answerYes{See Appendix}
         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
     \answerTODO{}
         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
     \answerYes{See Appendix}
 \end{enumerate}


 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
 \begin{enumerate}
   \item If your work uses existing assets, did you cite the creators?
     \answerYes{See Experiments section.}
   \item Did you mention the license of the assets?
     \answerYes{See Experiments section.}
   \item Did you include any new assets either in the supplemental material or as a URL?
     \answerNA{}
   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
     \answerNA{}
   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerNA{}
 \end{enumerate}


 \item If you used crowdsourcing or conducted research with human subjects...
 \begin{enumerate}
   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
     \answerNA{}
   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
     \answerNA{}
   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
     \answerNA{}
 \end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


